Distribution-Free Conformal Joint Prediction Regions for Neural Marked Temporal Point Processes

Sequences of labeled events observed at irregular intervals in continuous time are ubiquitous across various fields. Temporal Point Processes (TPPs) provide a mathematical framework for modeling these sequences, enabling inferences such as predicting the arrival time of future events and their associated label, called mark. However, due to model misspecification or lack of training data, these probabilistic models may provide a poor approximation of the true, unknown underlying process, with prediction regions extracted from them being unreliable estimates of the underlying uncertainty. This paper develops more reliable methods for uncertainty quantification in neural TPP models via the framework of conformal prediction. A primary objective is to generate a distribution-free joint prediction region for an event's arrival time and mark, with a finite-sample marginal coverage guarantee. A key challenge is to handle both a strictly positive, continuous response and a categorical response, without distributional assumptions. We first consider a simple but conservative approach that combines individual prediction regions for the event's arrival time and mark. Then, we introduce a more effective method based on bivariate highest density regions derived from the joint predictive density of arrival times and marks. By leveraging the dependencies between these two variables, this method excludes unlikely combinations of the two, resulting in sharper prediction regions while still attaining the pre-specified coverage level. We also explore the generation of individual univariate prediction regions for events' arrival times and marks through conformal regression and classification techniques. Moreover, we evaluate the stronger notion of conditional coverage. Finally, through extensive experimentation on both simulated and real-world datasets, we assess the validity and efficiency of these methods.

==> dl_book_commands.tex <==
% Source: https://github.com/goodfeli/dlbook_notation/blob/master/math_commands.tex

%%%%% NEW MATH DEFINITIONS %%%%%

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
%% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
%% Reference to an equation, upper case
%\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
%\def\rvepsilon{{\mathbf{\epsilon}}}
%\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vtheta{{\bm{\theta}}}
\def\vTheta{{\bm{\Theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> intervals_plots.tex <==
Retirer grid et couleur rouge. 

\clearpage
\thispagestyle{empty}
\newgeometry{top=0.5cm,bottom=0.5cm}

\textbf{LastFM}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/lastfm_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\textbf{MOOC}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/mooc_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\textbf{Github}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/github_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\textbf{Reddit}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/reddit_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\clearpage
\textbf{Retweets}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/retweets_filtered_short_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\clearpage
\textbf{Stack Overflow}

\begin{figure}[ht!]
        \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_1.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_2.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_3.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_4.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_5.png}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_6.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/intervals/stack_overflow_filtered_gru_cond-log-normal-mixture_temporal_with_labels_conformal_7.png}
    \end{subfigure}
    
\end{figure}





\restoregeometry

==> tabulars.tex <==
\clearpage
\thispagestyle{empty}
\newgeometry{top=0.5cm,bottom=0.5cm, left=0.5cm, right=0.5cm}

\begin{table}[h!]
\setlength\tabcolsep{1.5pt}
\small
\caption{Average coverage and length of the prediction regions generated by the Naive, Naive-C, HDR and C-HDR methods for various models and datasets.}
\begin{tabular}{cccccccc}
\toprule
                           & \multicolumn{7}{c}{Coverage} \\
                           & C-ConstAll & C-ConstAPS & C-CQRAll & Naive & C-Naive &   HDR & C-HDR \\
\midrule
        ('CLNM', 'LastFM') &      0.839 &      0.874 &    0.839 & 0.506 &   0.874 & 0.529 & 0.839 \\
          ('CLNM', 'MOOC') &       0.81 &       0.85 &    0.812 & 0.637 &   0.814 & 0.708 & 0.824 \\
        ('CLNM', 'Github') &      0.895 &      0.895 &    0.737 & 0.474 &   0.842 & 0.474 & 0.842 \\
        ('CLNM', 'Reddit') &      0.833 &      0.814 &     0.84 & 0.347 &   0.809 &  0.73 & 0.826 \\
      ('CLNM', 'Retweets') &      0.792 &      0.786 &    0.779 &  0.43 &   0.788 & 0.525 & 0.793 \\
('CLNM', 'Stack Overflow') &      0.801 &      0.828 &    0.803 & 0.619 &   0.847 & 0.693 &  0.82 \\
         ('THP', 'LastFM') &      0.839 &      0.862 &    0.839 & 0.494 &   0.862 & 0.494 & 0.793 \\
           ('THP', 'MOOC') &       0.81 &      0.847 &     0.81 & 0.809 &   0.848 & 0.697 & 0.666 \\
         ('THP', 'Github') &      0.895 &      0.947 &    0.895 & 0.368 &   0.947 & 0.368 & 0.579 \\
         ('THP', 'Reddit') &      0.833 &      0.823 &    0.833 & 0.133 &   0.823 & 0.314 & 0.498 \\
       ('THP', 'Retweets') &      0.792 &      0.792 &    0.792 & 0.356 &   0.793 &  0.48 & 0.746 \\
 ('THP', 'Stack Overflow') &      0.801 &      0.826 &    0.801 & 0.402 &   0.826 & 0.421 & 0.788 \\
\bottomrule
\toprule
                           & \multicolumn{7}{c}{Length} \\
                           & C-ConstAll & C-ConstAPS & C-CQRAll & Naive & C-Naive &   HDR &  C-HDR \\
\midrule
        ('CLNM', 'LastFM') &      8.054 &        6.7 &    8.083 & 0.734 &   \textbf{6.675} & 0.377 & 33.723 \\
          ('CLNM', 'MOOC') &      0.343 &      2.765 &    0.956 & 0.566 &   2.281 & 0.054 &  \textbf{0.255} \\
        ('CLNM', 'Github') &     16.299 &     10.622 &    8.046 & 1.608 &   5.968 & 1.197 &  \textbf{4.507} \\
        ('CLNM', 'Reddit') &     40.411 &     34.417 &   36.916 &   3.6 &  30.713 & 2.351 &  \textbf{6.025} \\
      ('CLNM', 'Retweets') &      6.793 &      6.712 &     \textbf{6.04} & 1.612 &   \textbf{6.042} & 1.932 &  6.465 \\
('CLNM', 'Stack Overflow') &      6.051 &       2.41 &    5.978 & 1.087 &   2.194 & 1.065 &  \textbf{1.653} \\
         ('THP', 'LastFM') &      8.054 &      9.805 &    8.054 & 1.093 &  10.068 & 0.961 &  \textbf{4.684} \\
           ('THP', 'MOOC') &      0.343 &      2.233 &    0.343 & 0.329 &   2.243 & 0.292 &  \textbf{0.255} \\
         ('THP', 'Github') &     16.299 &     14.468 &   16.299 & 0.788 &  14.468 & 0.761 &   3.85 \\
         ('THP', 'Reddit') &     40.411 &     28.739 &   40.411 & 0.182 &  28.735 & 0.165 &  1.647 \\
       ('THP', 'Retweets') &      6.793 &      6.724 &    6.799 & 0.888 &   6.729 & 1.328 &  5.761 \\
 ('THP', 'Stack Overflow') &      6.051 &      2.147 &    6.051 & 0.436 &   2.144 & 0.412 &  2.329 \\
\bottomrule
\toprule
                           & \multicolumn{7}{c}{WSC} \\
                           & C-ConstAll & C-ConstAPS & C-CQRAll & Naive & C-Naive &   HDR & C-HDR \\
\midrule
        ('CLNM', 'LastFM') &        0.6 &      0.857 &      0.9 & 0.333 &    0.75 &   0.4 & 0.818 \\
          ('CLNM', 'MOOC') &      0.776 &      0.826 &    0.843 & 0.667 &   0.836 & 0.623 & 0.803 \\
        ('CLNM', 'Github') &        1.0 &        1.0 &      1.0 &   0.4 &    0.75 & 0.667 &   1.0 \\
        ('CLNM', 'Reddit') &      0.652 &      0.595 &    0.679 &  0.06 &   0.568 &  0.75 & \textbf{0.868} \\
      ('CLNM', 'Retweets') &      0.685 &      0.766 &    0.795 & 0.403 &   0.795 & 0.482 & 0.748 \\
('CLNM', 'Stack Overflow') &      0.609 &      0.732 &    0.696 & 0.538 &   \textbf{0.807} & 0.716 & 0.758 \\
         ('THP', 'LastFM') &        1.0 &        1.0 &    0.875 &   0.4 &   0.857 & 0.417 & 0.786 \\
           ('THP', 'MOOC') &      0.874 &      0.778 &    0.885 & 0.795 &   0.861 & 0.754 & 0.636 \\
         ('THP', 'Github') &        nan &        1.0 &      1.0 &   0.6 &     1.0 &  0.75 & 0.667 \\
         ('THP', 'Reddit') &       0.86 &      0.562 &     0.61 & 0.161 &   0.577 & 0.337 & 0.515 \\
       ('THP', 'Retweets') &      0.688 &      0.776 &    0.648 & 0.224 &   0.777 & 0.289 & 0.673 \\
 ('THP', 'Stack Overflow') &      0.703 &      0.808 &     0.69 &  0.28 &   0.816 & 0.277 & 0.746 \\
\bottomrule
\end{tabular}

\end{table}

\restoregeometry

==> temp.tex <==

As outlined in \cref{sec:problem_setup}, our objective is to develop a joint prediction region for the time and mark, ensuring the marginal coverage guarantee (\ref{eq:marginal_cov}).

In \cref{sec:naive}, we present a naive approach that achieves this by combining individual conformal prediction regions for the time and mark (see \cref{sec:individual}). However, this technique fails to generate complex regions that could represent the interdependencies between time and mark.

Despite the potential applications of multi-output prediction regions, the exploration of conformal methods for such regions remains underdeveloped.
With Marked Temporal Point Processes (MTPPs), the joint density over time and mark, conditional on the history, can be easily derived from the intensity function.
This renders density-based methods particularly appealing.
\cite{Lei2013-ol} proposed a density-based conformal approach based on density level sets where the density is estimated by kernel density estimation. However, this method is not applicable to estimation problems with covariates. Alternatively, \cite{Feldman2023-cc} proposed a method centered on multi-output quantile regression. Nonetheless, this method is less suited to MTPPs due to the absence of an inherent order in the marks, thereby undermining the effectiveness of quantile regression.

Thus, in \cref{sec:conformal_hdr}, we turn to producing predictive regions in the form of highest density regions using the method HPD-Split \citep{Izbicki2022-ru}. 
This approach, in contrast to the method of combining independent regions for time and mark, allows us to exclude improbable time-mark combinations, albeit with increased computational demands.


\dobox{using a generalization of method HPD-Split \citep{Izbicki2022-ru}}

\dobox{Nominal coverage level" vs empirical coverage rate}


% In the following, we suppose that an off-the-shelf MTPP model is trained on $\mathcal{D}_{\text{train}}$, yielding an estimate $\hat{f}(\tau_m,k_m|\mathcal{H}_{t_m})$, i.e. the conditional density of the last event for a new observation. Following the steps of split conformal prediction described in Section \ref{sec:split_conf}, we now present how to construct and combine the independent prediction regions  $\hat{R}_\tau(\mathcal{H}_{t_m})$ and $\hat{R}_k(\mathcal{H}_{t_m})$. 

% Having constructed $\hat{R}_\tau(\mathcal{H}_{t_m})$ and $\hat{R}_k(\mathcal{H}_{t_m})$ for a new observation $(\tau_m, k_m)$ at level $1-\nicefrac{\alpha}{2}$, we finally obtain a joint prediction region as $\hat R_{\tau, k}(\mathcal{H}_{t_m}) = \hat{R}_\tau(\mathcal{H}_{t_m}) \times \hat{R}_k(\mathcal{H}_{t_m})$ that is guaranteed to have marginal coverage of at least $1-\alpha$ according to proposition (\ref{eq:bound}). By construction, this approach generates equal size prediction intervals $\hat{R}_\tau(\mathcal{H}_{t_m})$ for each mark $k \in \hat{R}_k(\mathcal{H}_{t_m})$. Indeed, suppose for instance that we obtain $\hat{R}_k(\mathcal{H}_{t_m}) = \Set{k_1, k_3}$ and $\hat{R}_\tau(\mathcal{H}_{t_m})= [2,3]$ for a new observation $(\tau_m,k_m)$. In this context, the joint prediction region would write $\hat{R}_{\tau,k}(\mathcal{H}_{t_m}) = \Set{k_1} \times [2,3] \cup \Set{k_3} \times [2,3]$. Illustration? \\

% Nonetheless, as shown by (\ref{eq:bound}), $\hat{R}_{\tau,k}(\mathcal{H}_{t_m})$ may actually emerge as over-conservative if $\hat{R}_\tau(\mathcal{H}_{t_m})$ and $\hat{R}(\mathcal{H}_{t_m})$ are constructed at nominal level $1-\nicefrac{\alpha}{2}$, despite meeting the desideratum in (\ref{eq:marginal_cov}). Moreover, by generating equal length intervals for each mark in $R_k(\mathcal{H}_{t_m}))$, we explicitly discard potential dependencies between arrival times and marks, which may further contribute to poor statistical efficiency. Consequently, we call this method Conformal Naive (C-Naive) and motivate in the next sub-section an alternative approach that takes the dependencies between arrival times and marks into account. 



% The approach of highest density regions (HDR, \cite{Hyndman1996-wx}) for a distribution $\hat{f}(\tau_m,k_m)$ at nominal coverage $1 - \alpha$ produces the region with highest density while achieving coverage of $1 - \alpha$, namely:
% \begin{equation}
%     \text{HDR}(1 - \alpha) = \Set{(\tau_m', k_m')| \hat{f}(\tau_m',k_m') \geq z} \quad \text{where} \quad z = \text{sup}\Set{z' | \mathbb{P}(\hat{f}(\tau_m,k_m) \geq z') \geq 1 - \alpha}
% \end{equation}
% This is provably the smallest prediction region with coverage $1 - \alpha$.
% In the case of a conditional distribution, if $\hat{f}(\tau_m,k_m|\boldsymbol{h}_m)$ corresponds to the true joint density of $\tau_m,k_m$, the regions produced by HDR are the smallest regions that achieve conditional coverage (\ref{eq:cond_cov}) (TO DISCUSS).

% Taking $\hat{q}$ as the $1-\alpha$ empirical quantile of the $s_{\text{HPD}}$ scores evaluated on the observations in $\mathcal{D}_{\text{cal}}$, we set
% \begin{equation}
%     z = \text{sup}\Set{z'|\mathbb{P}(\hat{f}(\tau_m,k_m|\mathcal{H}_{t_m}) \geq z') \geq \hat{q}},  
% \end{equation}
% for a new observation $(\tau_m,k_m)$, and define the joint prediction region $\hat{R}_{\tau,k}(\mathcal{H}_{t_m})$ as the HDR with coverage at least $\hat{q}$, i.e.
% \begin{equation}
%     \hat{R}_{\tau,k}(\mathcal{H}_{t_m}) = \text{HDR}(\hat{q}) = \Set{(\tau_m', k_m')| \hat{f}(\tau_m',k_m'|\mathcal{H}_{t_m}) \geq z}. 
% \label{eq:r_hpd}
% \end{equation}
% As previously, we can show that this prediction region verifies the conformal guarantee at nominal level $1-\alpha$, i.e.:
% \begin{equation}
%     \mathbb{P}((\tau_m,k_m) \in \hat{R}_{\tau,k}(\mathcal{H}_{t_m})) = \mathbb{P}(s_{\text{HPD}}(\mathcal{H}_{t_m}, (\tau_m,k_m)) \leq \hat{q}) \geq 1 - \alpha.
% \end{equation}
% In the following, we will refer to this approach as Conformal HDR (C-HDR). If we had access to the true $f(\tau_m,k_m|\mathcal{H}_{t_m})$, we could instead select $z$ as 
% \begin{equation}
%      z = \text{sup}\Set{z'|\mathbb{P}(f(\tau_m,k_m|\mathcal{H}_{t_m}) \geq z') \geq 1-\alpha},
% \end{equation}
% and construct a joint prediction region for $(\tau_m, k_m)$ using (\ref{eq:r_hpd}) that would satisfy (\ref{eq:marginal_cov}). 
% \dobox{Motivation for conformal missing:

% For a new test sequence, ...

% After training, the neural MTTP model $\hat{f}(\tau,k|\boldsymbol{h}) = f(\tau,k|\boldsymbol{h}; \btheta)$ can be used for prediction tasks and  addressing queries such as: When is the next event likely to occur? What will be the type of the next event, given that it occurs at a certain time t? How long until an event of type k occurs? Recall that for mod   els that parametrize $\hat{\lambda}_k(t|\boldsymbol{h})$ or $\hat{\Lambda}_k(t|\boldsymbol{h})$, $\hat{f}(\tau,k|\boldsymbol{h})$ can be retrieved from (\ref{eq:joint_Lambda})

% We could extract prediction intervals or region with a prespecified coverage ...

% However, heuristic notion of uncertainty ....

% To construct $\hat{R}_{\tau}(\boldsymbol{h}_{n+1})$, $\hat{R}_{k}(\boldsymbol{h}_{n+1})$, and $\hat{R}_{\tau,k}(\boldsymbol{h}_{n+1})$, one could naively be tempted to directly use the estimate $\hat{f}(\tau,k|\boldsymbol{h})$ obtained from a trained MTPP model. However, due to model misspecification, or lack of training data, $\hat{f}(\tau,k|\boldsymbol{h})$ may be a poor approximation of the true unknown $f^\ast(\tau,k)$. Consequently, constructing prediction regions directly from the model's estimate won't provide any of the above statistical guarantees. Fortunately, we can leverage the sound framework of split conformal prediction \citep{papadopoulos2002inductive} to account for errors in the model, enabling us to build predictions regions that achieve marginal coverage in finite-sample. 
% }


The standard approach would be to naively extract prediction intervals or regions with a prespecified coverage.

However, due to model misspecification or lack of training data, $\hat{f}(\tau,k|\boldsymbol{h})$ may be a poor approximation of the true unknown $f^\ast(\tau,k)$. Consequently, constructing prediction regions directly from the model's estimate won't provide any finite-sample statistical guarantees.

Fortunately, we can leverage the sound framework of split conformal prediction \citep{papadopoulos2002inductive} to account for errors in the model, enabling us to build predictions regions that achieve marginal coverage in finite-sample. 

For a sequence $ \mathcal{S}_i \in \mathcal{D}^\ast$, let us now define the input-output pair $(\boldsymbol{h}_{i,m_i}, e_{i,m_i})$, where $e_{i,m_i} = (\tau_{i,m_i}, k_{i, m_i})$ is a bivariate output corresponding to the last event in $\mathcal{S}_i$, and $\boldsymbol{h}_{i,m_i}$ is its history embedding. 

\begin{comment}
Additionally, suppose that we have access to $\hat{f}((\tau_m,k_m)|\boldsymbol{h}_m)$ from a MTPP model trained on the observations in $\mathcal{D}$, i.e. an estimate of the distribution of the last event of a given sequence $\mathcal{S}$ conditional on the history. 


From $\hat{f}((\tau_m,k_m)|\boldsymbol{h}_m)$, we seek to construct independent prediction regions $\hat{R}_{\tau}(\boldsymbol{h}_m) \subseteq \R^+$ and $\hat{R}_{k}(\boldsymbol{h}_m) \subseteq \K$, respectively for the inter-arrival time $\tau^{n+1}_m$ and mark $k^{n+1}_m$ of a new observation $e_m^{n+1}$ drawn exchangeably from the process.
\end{comment}

\begin{comment}
Nevertheless, we are currently lacking a key ingredient to carry out the above steps: How to obtain an estimate $\hat{f}(e_m|\mathcal{H}_{t_{m}})$ upon which split conformal prediction can operate? We leverage in the next section the framework of Marked Temporal Point Processes (MTPP) \citep{Daley} that offers principled approaches to model sequences of events in continuous time.  

accomplishes that by first splitting the data into two non-overlapping parts $\mc{D} = \mc{D}_{\text{train}} \cup \mc{D}_{\text{cal}}$.
Based on $\mc{D}_{\text{train}}$, a heuristic notion of uncertainty is created through a (non-conformity) score function $s(x,y) \in \mathbb{R}$, which assigns larger scores to worse agreement between $x$ and $y$.
Then, scores $S_i = s(X_i,Y_i)$ are computed using $\mc{D}_{\text{cal}}$ and the empirical quantile of the scores is defined by $\hat{q} = \text{Quantile}(1 - \alpha; \Set{S_i}_{i=1}^{|\mc{D}_{\text{cal}}|} \cup \Set{\infty})$.
Finally, prediction sets are created for new examples based on $\hat{q}$:
\[
\hat{R}(X_{n+1}) = \{y: s(X_{n+1}, y) \leq \hat{q}\} 
\]
The marginal ﬁnite-sample coverage is due to the quantile lemma, which states that if $S_1, \dots, S_n, S_{n+1}$ are exchangeable random variables, then for any miscoverage $\alpha \in (0, 1)$, we have
\[
\mathbb{P}\left\{ S_{n+1} \leq \text{Quantile}\left(1 - \alpha; \{S_i\}_{i=1}^n \cup \{\infty\}\right) \right\}  \leq 1 - \alpha.
\]

If ties between $S_1, \dots, S_n, S_{n+1}$ occur with probability zero, then the above probability is upper bound by $1 - \alpha + \frac{1}{n+1}$.
Let $\mathcal{D} = \{(X_i, Y_i)\}_{i=1}^n$ denote a dataset composed of $n$ i.i.d. (or more generally, exchangeable) pairs $(X_i, Y_i) \sim P$ for a distribution $P$ on $\mathcal{X} \times \mathcal{Y}$.
For a new i.i.d. pair $(X_{n+1}, Y_{n+1})$ and a miscoverage level $\alpha \in (0, 1)$, we want to generate a distribution-free prediction set $\hat{R}(X_{n+1}) \subseteq \mathcal{Y}$ with marginal ﬁnite-sample coverage, i.e. 
\begin{equation}
\label{sec:conformal_guarantee}
    \mathbb{P}(Y_{n+1} \in \hat{R}(X_{n+1})) \geq 1 - \alpha,
\end{equation}
for any distribution $P$.
Given a dataset of $n$ realizations $\{\mathcal{S}_i\}_{i=1}^n$ drawn exchangeably from a (unknown) ground-truth 
MTPP, each containing $m_i$ events, we wish to construct an informative prediction set $\hat{R}_{\tau,k}(X_{n+1}) \subseteq \mathbb{K} \times \R^+$ for the last event of a new realization $\mathcal{S}_{n+1}$ that achieves finite-sample coverage. Following the approach of \cite{Stankeviciute2021-ay} in the context of time series, we construct a dataset of exchangeable pairs $(X_i, Y_i)_{i=1}^n$ where $(X_i, Y_i)=(\mathcal{H}^i_{t_{m_i}}, e^i_{m_i} = (\tau^{i}_{m_{i}}, k^{i}_{m_{i}}))$, i.e., for a given sequence $\mathcal{S}_i$, $Y_i$ corresponds to the last event $e^i_{m_i}$, and $X_i$ is the observed history $\mathcal{H}^i_{t_{m_i}}$ until time $t_{m_i}$.

To achieve this goal, we aim to design conformal methods for the joint distribution of the time and mark.
By the quantile lemma, these methods achieve finite-sample coverage:
\begin{equation}
    \mathbb{P}(Y_{n+1} \in \hat{R}_{\tau,k}(X_{n+1})) = \mathbb{P}((\tau_m, k_m) \in \hat{R}_{\tau,k}(\mathcal{H}_{t_m})) \geq 1 - \alpha,
\label{eq:marginal_cov}
\end{equation}
where, for brevity of notations, we define $\mathcal{H}_{t_m} = \mathcal{H}^{n+1}_{t^_m}$, $\tau_{m} = \tau^{n+1}_m$ and $k_m = k^{n+1}_m$.
Additionally, these methods should produce prediction sets that are informative, i.e., they should approximate conditional coverage:
\begin{equation}
    \mathbb{P}(Y_{n+1} \in \hat{R}_{\tau,k}(X_{n+1}) \mid X_{n+1} = x) \approx 1 - \alpha \quad \forall x \in \mc{X}.
\label{eq:cond_cov}
\end{equation}
Following the conformal procedure described in section \ref{sec:split_conformal}, we start by randomly partitioning $\mathcal{D}$ into $\mathcal{D}_{\text{train}}$, $\mathcal{D}_{\text{cal}}$ and $\mathcal{D}_\text{test}$ non-overlapping sets. Then, an estimate of the unknown ground-truth 
$f^\ast(\tau,k)$ can be obtained by training any of-the-shelf MTPP model on $\mathcal{D}_{\text{train}}$ using, for instance, the objective in (\ref{eq:nll}). After training, we can exploit the resulting model estimate $\hat{f}^\ast(\tau,k)$ to make prediction of new events. We give an overview of several of these available MTPP models in section \ref{sec:baselines}. However, the estimate $\hat{f}^\ast(\tau,k)$ may be a poor approximation of $f^\ast(\tau,k)$, therefore lacking the statistical guarantees of (\ref{eq:marginal_cov}) and (\ref{eq:cond_cov}). In the next section, we leverage two conformal approaches to account for errors in $\hat{f}^\ast(\tau,k)$, thereby enabling finite-sample coverage of new observations.  
\end{comment}




 \begin{comment}
\textbf{Neural Temporal Point Processes.} To capture complex event dependencies, the framework of neural TPPs \citep{SchurSurvey} integrates neural network components into model design, thereby enabling flexible parametrizations. Usually, a neural MTPP model can be decomposed into three main components: (1) An \textit{event encoder} that generates a representation $\boldsymbol{e}_i \in \mathbb{R}^{d_e}$ for each event $e_i \in \mathcal{S}$, (2) a \textit{history encoder} that creates a compact history embedding $\boldsymbol{h}_i \in \mathbb{R}^{d_h}$ of the history $\mathcal{H}_{t_i}$ of event $e_i$, and (3) a \textit{decoder} that parametrizes a function characterizing the MTPP (e.g. $\lambda_k^\ast(t))$ from $\boldsymbol{h}_i$. 
\end{comment}

\begin{comment}
\subsection{Split Conformal Prediction}
\label{sec:split_conformal}

Let $\mathcal{D} = \{(X_i, Y_i)\}_{i=1}^n$ denote a dataset composed of $n$ i.i.d. (or more generally, exchangeable) pairs $(X_i, Y_i) \sim P$ for a distribution $P$ on $\mathcal{X} \times \mathcal{Y}$.
For a new i.i.d. pair $(X_{n+1}, Y_{n+1})$ and a miscoverage level $\alpha \in (0, 1)$, we want to generate a distribution-free prediction set $\hat{R}(X_{n+1}) \subseteq \mathcal{Y}$ with marginal ﬁnite-sample coverage, i.e. 
\begin{equation}
\label{sec:conformal_guarantee}
    \mathbb{P}(Y_{n+1} \in \hat{R}(X_{n+1})) \geq 1 - \alpha,
\end{equation}
for any distribution $P$.

Split conformal prediction accomplishes that by first splitting the data into two non-overlapping parts $\mc{D} = \mc{D}_{\text{train}} \cup \mc{D}_{\text{cal}}$.
Based on $\mc{D}_{\text{train}}$, a heuristic notion of uncertainty is created through a (non-conformity) score function $s(x,y) \in \mathbb{R}$, which assigns larger scores to worse agreement between $x$ and $y$.
Then, scores $S_i = s(X_i,Y_i)$ are computed using $\mc{D}_{\text{cal}}$ and the empirical quantile of the scores is defined by $\hat{q} = \text{Quantile}(1 - \alpha; \Set{S_i}_{i=1}^{|\mc{D}_{\text{cal}}|} \cup \Set{\infty})$.
Finally, prediction sets are created for new examples based on $\hat{q}$:
\[
\hat{R}(X_{n+1}) = \{y: s(X_{n+1}, y) \leq \hat{q}\} 
\]


The marginal ﬁnite-sample coverage is due to the quantile lemma, which states that if $S_1, \dots, S_n, S_{n+1}$ are exchangeable random variables, then for any miscoverage $\alpha \in (0, 1)$, we have
\[
\mathbb{P}\left\{ S_{n+1} \leq \text{Quantile}\left(1 - \alpha; \{S_i\}_{i=1}^n \cup \{\infty\}\right) \right\}  \geq 1 - \alpha.
\]

If ties between $S_1, \dots, S_n, S_{n+1}$ occur with probability zero, then the above probability is upper bound by $1 - \alpha + \frac{1}{n+1}$.

\end{comment}



\subsection{Conditional independence assumption (incomplete)}
\label{sec:cindep}

\dobox{ (RI)
Although I think what you wrote is correct, it is still not clear to me
if the second assumption is reasonable.
May construction, the HDR for $(k,\tau)$ is the smallest prediction set for this vector, so the conclusion 
that
$\text{HDR}_k(\hat{q}_k) \times \text{HDR}_\tau(\hat{q}_\tau) \subseteq \text{HDR}_{k,\tau}(\hat{q}_{k,\tau})$ is weird to me.

Maybe we could instead use the fact that, if the joint density factors, 
$$P(f(k,\tau) 
\geq z_{\hat{q}_{k}}z_{\hat{q}_{\tau}})\geq P(f(k)\geq z_{\hat{q}_k})P(f(\tau)\geq z_{\hat{q}_\tau}),$$
and therefore 
if we set the cutoffs so that $P(f(k)\geq z_{\hat{q}_k})=P(f(\tau)\geq z_{\hat{q}_\tau})=\sqrt{1-\alpha}$,
we can use $z_{\hat{q}_{k}}z_{\hat{q}_{\tau}}$
as the cutoff for the joint set (this will be a conservative set though, and I'm not sure if we would gain something from it). 
}

\dobox{(SBT) Thanks. I was wondering if we could say anything interesting when comparing joint HDR under a factorizable density compared to independent HDR for $\tau$ and independent HDR for $k$(i.e. APS). }

Some existing neural TPP models makes the following assumption: $ f(k, \tau |\bm{h}) = f(k|\bm{h}) \times f(t|\bm{h})$. Can we relate the individual HPDsplit regions to the joint HPDsplit region or say anything else interesting in this case? (There isn't a simple relationship between the quantile of $Z_1 \times Z_2$ to the quantile of $Z_1$ and the quantile of $Z_2$)



Let
\begin{align*}
    \text{HDR}_k(\hat{q}_k) &= \Set{ k : f(k) \geq z_{\hat{q}_k}} \\
    \text{HDR}_\tau(\hat{q}_\tau) &= \Set{ \tau : f(\tau) \geq z_{\hat{q}_\tau}} \\
    \text{HDR}_{k,\tau}(\hat{q}_{k,\tau}) &= \Set{ k, \tau : f(k, \tau) \geq z_{\hat{q}_{k,\tau}}} \\
    z_{\hat{q}_k} &= \text{sup}\Set{z' : P(f(k) \geq z') \geq \hat{q}_k} \\
    z_{\hat{q}_\tau} &= \text{sup}\Set{z' : P(f(\tau) \geq z') \geq \hat{q}_\tau} \\
    z_{\hat{q}_{k,\tau}} &= \text{sup}\Set{z' : P(f(k, \tau) \geq z') \geq \hat{q}_{k,\tau}} \\
\end{align*}

We assume that:
\begin{itemize}
    \item The density is factorizable: $f(k, \tau) = f(k) f(\tau)$.
    \item The product of the thresholds of HDR on the marginal densities is larger than the threshold of HDR on the joint density: $z_{\hat{q}_k} z_{\hat{q}_\tau} \geq z_{\hat{q}_{k,\tau}}$.
\end{itemize}

To better understand the second assumption, we can have for example $\hat{q}_k = \hat{q}_\tau = 1 - \nicefrac{\alpha}{2}$. Then $(1 - \nicefrac{\alpha}{2})^2 = 1 - \alpha + \nicefrac{\alpha^2}{4} \geq 1 - \alpha$.

We consider the prediction region defined by the cartesian product of HDR on the marginal densities:
\begin{align*}
    \text{HDR}_k(\hat{q}_k) \times \text{HDR}_\tau(\hat{q}_\tau) &= \Set{k, \tau : f(k) \geq z_{\hat{q}_k} \wedge f(\tau) \geq z_{\hat{q}_\tau}} \\
\end{align*}

We have:
\begin{align*}
    &f(k) \geq z_{\hat{q}_k} \wedge f(\tau) \geq z_{\hat{q}_\tau} \\
    \Longrightarrow & f(k) f(\tau) \geq z_{\hat{q}_k} z_{\hat{q}_\tau} & \quad\text{(Because the densities and thresholds are $\geq 0$)} \\
    \Longrightarrow & f(k, \tau) \geq z_{\hat{q}_{k,\tau}} & \quad\text{(Using the two assumptions)} \\
\end{align*}

We conclude that $\text{HDR}_k(\hat{q}_k) \times \text{HDR}_\tau(\hat{q}_\tau) \subseteq \text{HDR}_{k,\tau}(\hat{q}_{k,\tau})$. How is that useful?



\subsection{Conformal prediction methods}

%\dobox{Time: CQR, CQR-left, conditional histogram, HPDsplit}
%\dobox{APS, RAPS, PMF alone} 

We first focus on creating distinct univariate prediction regions for the event arrival time and the event mark of new test inputs. This is achieved through the application of conformal regression and classification techniques, as detailed in Section \ref{sec:individual}. Additionally, we explore CP methods for constructing bivariate prediction regions for both the event arrival time and its associated mark, as described in Section \ref{sec:joint}. We provide a summary of these methods below.




\textbf{Baselines to build prediction regions for the time.} To build a prediction region $\hat{R}_\tau(\boldsymbol{h}_{n+1})$ for $\tau_{n+1}$, we consider C-QR and C-QRL, which prediction regions are respectively obtained by (\ref{eq:R_CQR}) and (\ref{eq:R_CQRL}). Additionally, we focus on a marginal version of the C-HDR approach of Section \ref{sec:joint}, referred to as C-HDR-T, that constructs a prediction region $\hat{R}_\tau(\boldsymbol{h}_{n+1})$ directly from $\hat{f}(\tau|\boldsymbol{h}_{n+1})$, i.e. 
\begin{equation}
    \hat{R}_{\tau}(\boldsymbol{h}_{n+1}) = \Set{\tau| \hat{f}(\tau)|\boldsymbol{h}_{n+1}) \geq z_{\hat{q}}} \text{ where } z_{\hat{q}} = \text{sup}\Set{z' | \mathbb{P}(\hat{f}(\tau|\boldsymbol{h}_{n+1}) \geq \hat{q}}, 
\end{equation}
where $\hat{q}$ is the adjusted $1-\alpha$ quantile of the following non-conformity scores evaluated on the calibration set:
\begin{equation}
    s_{\text{C-HDR-T}}(\boldsymbol{h}, \tau) = \int_{\Set{\tau'|\hat{f}(\tau' |\boldsymbol{h}) \geq \hat{f}(\tau|\boldsymbol{h})}} \hat{f}(\tau'|\boldsymbol{h})d\tau
\end{equation}
As baselines for comparison, we also consider the non-conformal variants of these aforementioned methods, obtained by naively substituting the model estimate in the corresponding oracle prediction region. We denote these methods as Naive QR (N-QR), Naive QRL (N-QRL) and Naive HDR-T (N-HDR-T), for which we respectively define a prediction region for $\tau_{n+1}$ as: 
\begin{equation}
    \hat{R}_{\tau,\text{N-QR}}(\boldsymbol{h}_{n+1}) =[\hat{Q}_\tau(\alpha|\boldsymbol{h}_{n+1}),\hat{Q}_\tau(1-\alpha|\boldsymbol{h}_{n+1})],
\end{equation}
\begin{equation}
    \hat{R}_{\tau, \text{N-QRL}}(\boldsymbol{h}_{n+1}) = [0,\hat{Q}_\tau(1-\alpha|\boldsymbol{h}_{n+1})],
\end{equation}
\begin{equation}
    \hat{R}_{\tau,\text{N-HDR-T}}(\boldsymbol{h}_{n+1}) = \Set{\tau| \hat{f}(\tau|\boldsymbol{h}_{n+1}) \geq z_{1-\alpha}} \text{ where } z_{1-\alpha} = \text{sup}\Set{z' | \mathbb{P}(\hat{f}(\tau|\boldsymbol{h}_{n+1}) \geq 1 - \alpha}. 
\end{equation}
In order to measure the benefits of producing prediction intervals based on TPPs predictions, we further propose an additional conformal approach as a baseline.
The nonconformity score is plainly defined as the input inter-arrival time $s_\text{C}(\boldsymbol{h}, \tau) = \tau$ and the prediction region is $\hat{R}_\tau(\boldsymbol{h}_{n+1}) = [0, \hat{q}]$. This approach, that we denote as C-CONST, could be considered as the most simple conformal baseline, with prediction intervals that are by definition independent of the history $\boldsymbol{h}$. \\



\textbf{Baselines to build prediction regions for the mark.} To construct $\hat{R}_k(\boldsymbol{h}_{n+1})$ for $k_{n+1}$, we consider the C-RAPS approach in (\ref{eq:r_k}), and compare it to the unreguralized C-APS algorithm presented in \citep{Romano2020-ed}. Here also, we consider as baselines their non-conformal variants, denoted as Naive APS (N-APS) and Naive RAPS (N-RAPS), obtained by naively substituting the model estimate $\hat{p}(k)$ into the oracle prediction region, i.e.
\begin{equation}
    \hat{R}_{k,\text{N-APS}}(\boldsymbol{h}_{n+1})  = \Set{k' \in \mathbb{K}: s_{\text{APS}}(\boldsymbol{h}_{n+1}, k') \leq 1- \alpha},
\label{eq:oracle_RAPS}
\end{equation}
\begin{equation}
    \hat{R}_{k,\text{N-RAPS}}(\boldsymbol{h}_{n+1})  = \Set{k' \in \mathbb{K}: s_{\text{RAPS}}(\boldsymbol{h}_{n+1}, k') \leq 1- \alpha}. 
\label{eq:oracle_RAPS}
\end{equation}
Moreover, we ponder the simple C-PROB conformal baseline introduced in \citep{Angelopoulos2021-rc}, whose nonconformity score is plainly defined in terms of the estimated probability of the ground-truth mark:   
\begin{equation}
    s_{\text{PROB}}(\boldsymbol{h}, k) = 1 - \hat{p}(k|\boldsymbol{h}), 
\end{equation}
leading to the following prediction regions after computing $\hat{q}$ using (\ref{eq:qhat}): 
\begin{equation}
    \hat{R}(\boldsymbol{h}_{n+1}) = \Set{k' \in \K: \hat{p}(k'|\boldsymbol{h}) \geq 1 - \hat{q}}. 
\end{equation}



\textbf{Baselines to build joint prediction regions.} We compare the conformal methods highlighted in Section \ref{sec:joint} to build joint prediction regions $\hat{R}_{\tau,k}(\boldsymbol{h}_{n+1})$ for the bivariate output $(\tau_{n+1}, k_{n+1})$. For the approach based on the combination of independent regions of Section \ref{sec:naive}, we design two variants based on how $\hat{R}_\tau(\boldsymbol{h}_{n+1})$ and $\hat{R}_k(\boldsymbol{h}_{n+1})$ are individually constructed. The first one, denoted C-QRL-RAPS, employs C-QRL and C-RAPS to build $\hat{R}_\tau(\boldsymbol{h}_{n+1})$ and $\hat{R}_k(\boldsymbol{h}_{n+1})$, respectively. The second, C-HDR-RAPS, also relies on C-RAPS to build $\hat{R}_k(\boldsymbol{h}_{n+1})$, but leverages instead C-HDR-T for $\hat{R}_\tau(\boldsymbol{h}_{n+1})$. We benchmark these two methods against the C-HDR approach of Section \ref{sec:conformal_hdr}. As before, each of these methods is compared to their non-conformal variant, which will be referred to as N-QRL-RAPS, N-HDR-RAPS, and N-HDR, respectively. 


% \begin{itemize}
%     \item Coverage: C-HDR for THP does not achieve coverage on MOOC. Otherwise all conformal methods satisfy marginal coverage, contrary to the base models. 
%     \item WSC/other conditional coverage metrics: Although conformal methods do not systematically satisfy WSC, they perform better than non-conformal methods (except HPD-split for THP on MOOC). No clear winner among CQR, Const, or HPD-split clearly stands out. 
%     \item Length: In terms of relative length, HPD-split appears to be generally on par or worse compared to the other conformal methods. This can be mainly explained by the high adaptiveness of the algorithm, which can generate very large $\hat{R}_\tau(\boldsymbol{h}_{n+1})$ for a $\tau_{n+1}$ if $\hat{q} \simeq 1$, and if the estimated $\hat{f}(\tau|\boldsymbol{h}_{n+1})$ is highly skewed, which frequently occurs in datasets such as LastFM. The Constant and CQR methods are usually on par, at the exception of the MOOC dataset where Const, despite its simplicity, leads to very narrow prediction regions. Comparing CQR to N-CQR, we see that the interval size can be mostly attributed to the $\hat{Q}(1-\alpha)$, which can take on large value if the estimated $\hat{f}(\tau|\boldsymbol{h}_{n+1})$ is highly skewed for certain test points.  
% \end{itemize}

% \begin{itemize}
%     \item Marginal coverage: non-conformal methods are already quite well calibrated but sometimes undercover. Conformal methods always achieve coverage, with overcoverage for APS.
%     \item Conditional coverage: methods that have a good marginal coverage achieve a good conditional coverage.
%     \item Length: RAPS has smaller lengths than APS, which is not surprising.
% \end{itemize}
